Mean proper motions, space orbits and velocity dispersion profiles of Galactic globular clusters derived from Gaia DR2 data

We have derived the mean proper motions and space velocities of 154 Galactic globular clusters and the velocity dispersion profiles of 141 globular clusters based on a combination of Gaia DR2 proper motions with ground-based line-of-sight velocities. Combining the velocity dispersion profiles derived here with new measurements of the internal mass functions allows us to model the internal kinematics of 144 clusters, more than 90% of the currently known Galactic globular cluster population. We also derive the initial cluster masses by calculating the cluster orbits backwards in time applying suitable recipes to account for mass loss and dynamical friction. We find a correlation between the stellar mass function of a globular cluster and the amount of mass lost from the cluster, pointing to dynamical evolution as one of the mechanisms shaping the mass function of stars in clusters. The mass functions also show strong evidence that globular clusters started with a bottom-light initial mass function. Our simulations show that the currently surviving globular cluster population has lost about 80% of its mass since the time of formation. If globular clusters started from a log-normal mass function, we estimate that the Milky Way contained about 500 globular clusters initially, with a combined mass of about $2.5 \cdot 10^8$ $M_\odot$. For a power-law initial mass function, the initial mass in globular clusters could have been a factor of three higher.

==> propermotion_tab.tex <==
\begin{table*}
\caption{Derived proper motions of Galactic globular clusters. For each cluster, the Table gives the name of the cluster, the right ascension and declination, the distance from the Sun, the mean radial velocity of the cluster and its $1\sigma$ error, the proper motion in right ascension and declination and the correlation $\rho$ between both parameters.}

\begin{tabular}{lrrr@{}lr@{}lr@{}lr@{}lr}
\hline
 & & & & & & & & \\[-0.3cm]
\multirow{2}{*}{Name} &  \multicolumn{1}{c}{RA} & \multicolumn{1}{c}{DEC} & \multicolumn{2}{c}{$R_\odot$} & \multicolumn{2}{c}{$R_V$} &\multicolumn{2}{c}{$\mu_\alpha \cos \delta$} & \multicolumn{2}{c}{$\mu_\delta$} & \multirow{2}{*}{$\rho_{\mu_\alpha \mu_\delta}$}  \\
 &  \multicolumn{1}{c}{$[^0]$} & \multicolumn{1}{c}{$[^0]$} & \multicolumn{2}{c}{[kpc]} & \multicolumn{2}{c}{[km/sec]} & \multicolumn{2}{c}{[mas/yr]} & \multicolumn{2}{c}{[mas/yr]} & \\[+0.1cm]
\hline
 & & & & & & & & \\[-0.3cm]
NGC 104 &   6.023625 & -72.081276 &    4.43 $\pm \;$ &   0.04 &  -17.17 $\pm \;$ &   0.17 &    5.25 $\pm \;$ &   0.01 &   -2.53 $\pm \;$ &   0.01 &   -0.03 \\
NGC 288 &  13.188500 & -26.582611 &    9.95 $\pm \;$ &   0.37 &  -44.84 $\pm \;$ &   0.12 &    4.22 $\pm \;$ &   0.01 &   -5.64 $\pm \;$ &   0.01 &    0.31 \\
NGC 362 &  15.809416 & -70.848778 &    9.33 $\pm \;$ &   0.20 &  223.32 $\pm \;$ &   0.28 &    6.70 $\pm \;$ &   0.01 &   -2.51 $\pm \;$ &   0.01 &   -0.09 \\
Whiting 1 &  30.737499 &  -3.252777 &   30.10 $\;\;\;\;$ &  & -129.20 $\pm \;$ &   2.32 &    0.55 $\pm \;$ &   0.12 &   -4.35 $\pm \;$ &   0.09 &   -0.11 \\
NGC 1261 &  48.067543 & -55.216224 &   15.49 $\;\;\;\;$ &  &   71.46 $\pm \;$ &   0.25 &    1.58 $\pm \;$ &   0.02 &   -2.08 $\pm \;$ &   0.02 &    0.20 \\
Pal 1 &  53.333499 &  79.581054 &   11.10 $\;\;\;\;$ &  &  -74.90 $\pm \;$ &   0.41 &   -0.14 $\pm \;$ &   0.07 &   -0.01 $\pm \;$ &   0.08 &    0.07 \\
AM 1 &  58.759586 & -49.615276 &  123.00 $\;\;\;\;$ &  &  104.00 $\pm \;$ &  20.00 &    0.38 $\pm \;$ &   0.14 &   -0.46 $\pm \;$ &   0.18 &   -0.09 \\
Eridanus   &  66.185417 & -21.186943 &   90.10 $\;\;\;\;$ &  &  -23.75 $\pm \;$ &   1.04 &    0.28 $\pm \;$ &   0.20 &    0.21 $\pm \;$ &   0.24 &   -0.37 \\
Pal 2 &  71.524620 &  31.381500 &   27.20 $\;\;\;\;$ &  & -135.46 $\pm \;$ &   1.59 &    0.54 $\pm \;$ &   0.13 &   -1.43 $\pm \;$ &   0.08 &    0.12 \\
NGC 1851 &  78.528160 & -40.046555 &   11.42 $\pm \;$ &   0.18 &  320.23 $\pm \;$ &   0.20 &    2.12 $\pm \;$ &   0.02 &   -0.63 $\pm \;$ &   0.02 &   -0.18 \\
NGC 1904 &  81.044168 & -24.524481 &   13.27 $\;\;\;\;$ &  &  205.61 $\pm \;$ &   0.20 &    2.48 $\pm \;$ &   0.02 &   -1.61 $\pm \;$ &   0.02 &    0.02 \\
NGC 2298 & 102.247543 & -36.005306 &   10.80 $\;\;\;\;$ &  &  145.02 $\pm \;$ &   0.37 &    3.30 $\pm \;$ &   0.02 &   -2.20 $\pm \;$ &   0.02 &    0.08 \\
NGC 2419 & 114.535286 &  38.882442 &   83.18 $\;\;\;\;$ &  &  -20.88 $\pm \;$ &   0.30 &   -0.02 $\pm \;$ &   0.03 &   -0.56 $\pm \;$ &   0.02 &    0.10 \\
Pyxis   & 136.990833 & -37.221388 &   39.40 $\;\;\;\;$ &  &   40.37 $\pm \;$ &   0.19 &    1.01 $\pm \;$ &   0.04 &    0.15 $\pm \;$ &   0.05 &    0.17 \\
NGC 2808 & 138.012909 & -64.863495 &   10.15 $\pm \;$ &   0.15 &  103.79 $\pm \;$ &   0.28 &    1.01 $\pm \;$ &   0.01 &    0.28 $\pm \;$ &   0.01 &   -0.10 \\
E 3 & 140.237793 & -77.281890 &    8.09 $\;\;\;\;$ &  &    5.38 $\pm \;$ &   0.50 &   -2.66 $\pm \;$ &   0.03 &    7.07 $\pm \;$ &   0.03 &   -0.15 \\
Pal 3 & 151.382916 &   0.071666 &   92.50 $\;\;\;\;$ &  &   94.04 $\pm \;$ &   0.80 &   -0.03 $\pm \;$ &   0.23 &   -0.24 $\pm \;$ &   0.28 &   -0.59 \\
NGC 3201 & 154.403427 & -46.412476 &    4.61 $\pm \;$ &   0.18 &  494.41 $\pm \;$ &   0.15 &    8.34 $\pm \;$ &   0.01 &   -2.00 $\pm \;$ &   0.01 &    0.26 \\
Pal 4 & 172.320000 &  28.973583 &  103.00 $\;\;\;\;$ &  &   72.49 $\pm \;$ &   0.23 &   -0.34 $\pm \;$ &   0.08 &   -0.20 $\pm \;$ &   0.16 &   -0.64 \\
Crater   & 174.067500 & -10.877444 &  145.00 $\;\;\;\;$ &  &  148.41 $\pm \;$ &   0.82 &    0.61 $\pm \;$ &   0.63 &   -0.28 $\pm \;$ &   0.37 &   -0.10 \\
NGC 4147 & 182.526260 &  18.542638 &   18.20 $\;\;\;\;$ &  &  179.27 $\pm \;$ &   0.32 &   -1.70 $\pm \;$ &   0.03 &   -2.10 $\pm \;$ &   0.02 &   -0.26 \\
NGC 4372 & 186.439178 & -72.659004 &    5.85 $\pm \;$ &   0.33 &   75.43 $\pm \;$ &   0.27 &   -6.39 $\pm \;$ &   0.01 &    3.33 $\pm \;$ &   0.01 &    0.09 \\
Rup 106 & 189.667500 & -51.150277 &   21.20 $\;\;\;\;$ &  &  -38.24 $\pm \;$ &   0.27 &   -1.26 $\pm \;$ &   0.01 &    0.38 $\pm \;$ &   0.01 &    0.67 \\
NGC 4590 & 189.866577 & -26.744057 &   10.59 $\;\;\;\;$ &  &  -93.10 $\pm \;$ &   0.19 &   -2.75 $\pm \;$ &   0.01 &    1.79 $\pm \;$ &   0.01 &   -0.45 \\
NGC 4833 & 194.891342 & -70.876503 &    6.11 $\pm \;$ &   0.40 &  201.84 $\pm \;$ &   0.33 &   -8.35 $\pm \;$ &   0.01 &   -0.97 $\pm \;$ &   0.01 &    0.18 \\
NGC 5024 & 198.230209 &  18.168165 &   17.90 $\;\;\;\;$ &  &  -62.92 $\pm \;$ &   0.23 &   -0.12 $\pm \;$ &   0.01 &   -1.34 $\pm \;$ &   0.01 &   -0.45 \\
NGC 5053 & 199.112875 &  17.700250 &   17.20 $\;\;\;\;$ &  &   42.76 $\pm \;$ &   0.23 &   -0.36 $\pm \;$ &   0.02 &   -1.26 $\pm \;$ &   0.01 &   -0.35 \\
NGC 5139 & 201.696838 & -47.479584 &    5.21 $\pm \;$ &   0.06 &  234.08 $\pm \;$ &   0.20 &   -3.25 $\pm \;$ &   0.02 &   -6.74 $\pm \;$ &   0.02 &   -0.49 \\
NGC 5272 & 205.548416 &  28.377277 &    9.57 $\pm \;$ &   0.45 & -147.13 $\pm \;$ &   0.29 &   -0.13 $\pm \;$ &   0.02 &   -2.66 $\pm \;$ &   0.01 &   -0.05 \\
NGC 5286 & 206.611710 & -51.374249 &   11.27 $\pm \;$ &   0.79 &   62.30 $\pm \;$ &   0.42 &    0.20 $\pm \;$ &   0.02 &   -0.18 $\pm \;$ &   0.02 &   -0.04 \\
AM 4 & 209.090423 & -27.167499 &   32.20 $\;\;\;\;$ &  &  148.98 $\pm \;$ &   2.86 &   -1.07 $\pm \;$ &   0.86 &   -3.93 $\pm \;$ &   0.92 &   -0.29 \\
NGC 5466 & 211.363708 &  28.534445 &   16.90 $\;\;\;\;$ &  &  106.88 $\pm \;$ &   0.17 &   -5.40 $\pm \;$ &   0.01 &   -0.79 $\pm \;$ &   0.01 &    0.11 \\
NGC 5634 & 217.405125 &  -5.976416 &   27.20 $\;\;\;\;$ &  &  -16.21 $\pm \;$ &   0.51 &   -1.67 $\pm \;$ &   0.02 &   -1.55 $\pm \;$ &   0.02 &   -0.06 \\
NGC 5694 & 219.901199 & -26.538944 &   37.33 $\;\;\;\;$ &  & -139.37 $\pm \;$ &   0.42 &   -0.43 $\pm \;$ &   0.03 &   -1.07 $\pm \;$ &   0.03 &   -0.43 \\
IC 4499 & 225.076875 & -82.213694 &   18.20 $\;\;\;\;$ &  &   38.21 $\pm \;$ &   0.47 &    0.46 $\pm \;$ &   0.02 &   -0.50 $\pm \;$ &   0.02 &    0.13 \\
NGC 5824 & 225.994293 & -33.068222 &   31.80 $\;\;\;\;$ &  &  -25.92 $\pm \;$ &   0.47 &   -1.17 $\pm \;$ &   0.03 &   -2.23 $\pm \;$ &   0.02 &    0.03 \\
Pal 5 & 229.021875 &  -0.111611 &   23.20 $\;\;\;\;$ &  &  -58.47 $\pm \;$ &   0.21 &   -2.82 $\pm \;$ &   0.03 &   -2.63 $\pm \;$ &   0.03 &   -0.41 \\
NGC 5904 & 229.352083 & -21.010277 &   12.56 $\pm \;$ &   1.10 &  101.25 $\pm \;$ &   0.20 &   -5.42 $\pm \;$ &   0.01 &   -3.46 $\pm \;$ &   0.01 &   -0.19 \\
NGC 5927 & 229.638412 &   2.081028 &    7.55 $\pm \;$ &   0.16 &   53.55 $\pm \;$ &   0.20 &    4.06 $\pm \;$ &   0.01 &   -9.89 $\pm \;$ &   0.01 &   -0.14 \\
NGC 5946 & 232.002869 & -50.673031 &    8.44 $\pm \;$ &   0.37 & -104.26 $\pm \;$ &   0.30 &   -5.05 $\pm \;$ &   0.02 &   -3.20 $\pm \;$ &   0.02 &   -0.25 \\
NGC 5986 & 233.868835 & -50.659668 &   10.60 $\;\;\;\;$ &  &  137.89 $\pm \;$ &   1.32 &   -5.31 $\pm \;$ &   0.03 &   -1.67 $\pm \;$ &   0.03 &   -0.26 \\
NGC 6093 & 236.512496 & -37.786415 &    9.66 $\pm \;$ &   0.49 &  101.37 $\pm \;$ &   0.42 &   -4.19 $\pm \;$ &   0.02 &   -4.60 $\pm \;$ &   0.02 &   -0.30 \\
FSR 1716 & 242.625000 & -53.748888 &    7.50 $\;\;\;\;$ &  &  -31.03 $\pm \;$ &   0.64 &   -4.55 $\pm \;$ &   0.06 &   -8.53 $\pm \;$ &   0.05 &   -0.24 \\
Pal 14 & 242.752500 &  14.957777 &   71.00 $\;\;\;\;$ &  &   72.29 $\pm \;$ &   0.13 &   -0.48 $\pm \;$ &   0.07 &   -0.47 $\pm \;$ &   0.06 &    0.43 \\
Lynga 7 & 242.765213 & -55.317775 &    8.00 $\;\;\;\;$ &  &   20.50 $\pm \;$ &   1.65 &   -3.73 $\pm \;$ &   0.02 &   -7.06 $\pm \;$ &   0.02 &   -0.26 \\
NGC 6101 & 244.260040 & -22.976084 &    9.20 $\pm \;$ &   0.46 &   11.04 $\pm \;$ &   0.38 &   -2.93 $\pm \;$ &   0.03 &   -5.59 $\pm \;$ &   0.03 &   -0.13 \\
NGC 6139 & 245.896744 & -26.525749 &    1.98 $\pm \;$ &   0.04 &   71.04 $\pm \;$ &   0.08 &  -12.49 $\pm \;$ &   0.01 &  -18.99 $\pm \;$ &   0.01 &    0.02 \\
NGC 6121 & 246.450485 & -72.202194 &   16.07 $\;\;\;\;$ &  &  367.36 $\pm \;$ &   0.79 &    1.76 $\pm \;$ &   0.01 &   -0.21 $\pm \;$ &   0.01 &    0.06 \\
NGC 6171 & 246.807769 & -26.023500 &    8.90 $\;\;\;\;$ &  &  195.67 $\pm \;$ &   0.81 &   -1.74 $\pm \;$ &   0.03 &   -2.64 $\pm \;$ &   0.03 &   -0.03 \\
NGC 6144 & 246.918212 & -38.848747 &    9.88 $\pm \;$ &   0.88 &   24.82 $\pm \;$ &   0.89 &   -6.27 $\pm \;$ &   0.10 &   -2.66 $\pm \;$ &   0.09 &    0.03 \\
Ter 3 & 247.167000 & -35.353472 &    8.10 $\;\;\;\;$ &  & -135.73 $\pm \;$ &   0.56 &   -5.69 $\pm \;$ &   0.05 &   -1.72 $\pm \;$ &   0.04 &    0.17 \\
NGC 6205 & 248.132751 & -13.053778 &    5.91 $\pm \;$ &   0.41 &  -34.74 $\pm \;$ &   0.18 &   -1.93 $\pm \;$ &   0.01 &   -5.97 $\pm \;$ &   0.01 &   -0.03 \\
ESO 452-SC11   & 249.854166 & -28.399166 &    7.80 $\;\;\;\;$ &  &   16.75 $\pm \;$ &   0.39 &   -1.54 $\pm \;$ &   0.05 &   -6.36 $\pm \;$ &   0.04 &   -0.11 \\
NGC 5897 & 250.421814 &  36.459862 &    6.66 $\pm \;$ &   0.38 & -244.73 $\pm \;$ &   0.34 &   -3.16 $\pm \;$ &   0.01 &   -2.56 $\pm \;$ &   0.02 &    0.29 \\
NGC 6229 & 251.744958 &  47.527750 &   30.62 $\;\;\;\;$ &  & -138.30 $\pm \;$ &   0.75 &   -1.20 $\pm \;$ &   0.07 &   -0.45 $\pm \;$ &   0.07 &    0.18 \\
NGC 6218 & 251.809067 &  -1.948528 &    4.54 $\pm \;$ &   0.22 &  -41.37 $\pm \;$ &   0.18 &   -0.15 $\pm \;$ &   0.02 &   -6.76 $\pm \;$ &   0.02 &    0.47 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\contcaption{}
\begin{tabular}{lrrr@{}lr@{}lr@{}lr@{}lr}
\hline
 & & & & & & & & \\[-0.3cm]
\multirow{2}{*}{Name} &  \multicolumn{1}{c}{RA} & \multicolumn{1}{c}{DEC} & \multicolumn{2}{c}{$R_\odot$} & \multicolumn{2}{c}{$R_V$} &\multicolumn{2}{c}{$\mu_\alpha \cos \delta$} & \multicolumn{2}{c}{$\mu_\delta$} & \multirow{2}{*}{$\rho_{\mu_\alpha \mu_\delta}$}  \\
 &  \multicolumn{1}{c}{$[^0]$} & \multicolumn{1}{c}{$[^0]$} & \multicolumn{2}{c}{[kpc]} & \multicolumn{2}{c}{[km/sec]} & \multicolumn{2}{c}{[mas/yr]} & \multicolumn{2}{c}{[mas/yr]} & \\[+0.1cm]
\hline
 & & & & & & & & \\[-0.3cm]
FSR 1735 & 253.044174 & -47.058055 &    9.80 $\;\;\;\;$ &  &  -73.27 $\pm \;$ &   6.30 &   -3.73 $\pm \;$ &   0.28 &   -4.41 $\pm \;$ &   0.23 &   -0.04 \\
NGC 6235 & 253.355458 & -22.177444 &   13.52 $\;\;\;\;$ &  &  126.68 $\pm \;$ &   0.33 &   -3.95 $\pm \;$ &   0.05 &   -7.60 $\pm \;$ &   0.05 &    0.27 \\
NGC 6254 & 254.287720 &  -4.100306 &    5.19 $\pm \;$ &   0.16 &   74.30 $\pm \;$ &   0.24 &   -4.72 $\pm \;$ &   0.02 &   -6.54 $\pm \;$ &   0.02 &    0.28 \\
NGC 6256 & 254.885916 & -37.121388 &    6.40 $\;\;\;\;$ &  & -100.54 $\pm \;$ &   0.77 &   -3.66 $\pm \;$ &   0.14 &   -1.39 $\pm \;$ &   0.11 &   -0.00 \\
Pal 15 & 254.962500 &  -0.538888 &   79.43 $\;\;\;\;$ &  &   72.62 $\pm \;$ &   1.73 &   -0.67 $\pm \;$ &   0.07 &   -0.85 $\pm \;$ &   0.05 &    0.10 \\
NGC 6266 & 255.303329 & -30.113722 &    5.68 $\pm \;$ &   0.06 &  -74.48 $\pm \;$ &   0.66 &   -4.97 $\pm \;$ &   0.03 &   -2.92 $\pm \;$ &   0.03 &    0.22 \\
NGC 6273 & 255.657486 & -26.267971 &    7.94 $\pm \;$ &   0.46 &  145.29 $\pm \;$ &   0.54 &   -3.24 $\pm \;$ &   0.02 &    1.67 $\pm \;$ &   0.02 &    0.21 \\
NGC 6284 & 256.118791 & -24.764861 &   15.30 $\;\;\;\;$ &  &   30.00 $\pm \;$ &   0.66 &   -3.14 $\pm \;$ &   0.02 &   -2.01 $\pm \;$ &   0.02 &    0.24 \\
NGC 6287 & 256.288051 & -22.708361 &    9.40 $\;\;\;\;$ &  & -294.74 $\pm \;$ &   1.65 &   -4.92 $\pm \;$ &   0.04 &   -1.96 $\pm \;$ &   0.03 &    0.04 \\
NGC 6293 & 257.542500 & -26.582083 &    9.29 $\pm \;$ &   0.67 & -143.66 $\pm \;$ &   0.39 &    0.88 $\pm \;$ &   0.03 &   -4.30 $\pm \;$ &   0.02 &    0.17 \\
NGC 6304 & 258.634399 & -29.462028 &    5.88 $\pm \;$ &   0.42 & -108.83 $\pm \;$ &   0.41 &   -4.04 $\pm \;$ &   0.04 &   -1.01 $\pm \;$ &   0.04 &    0.21 \\
NGC 6316 & 259.155416 & -28.140111 &   11.60 $\;\;\;\;$ &  &   99.22 $\pm \;$ &   0.80 &   -5.00 $\pm \;$ &   0.06 &   -4.59 $\pm \;$ &   0.06 &    0.12 \\
NGC 6341 & 259.280762 &  43.135944 &    8.42 $\pm \;$ &   0.38 & -120.56 $\pm \;$ &   0.26 &   -4.93 $\pm \;$ &   0.02 &   -0.55 $\pm \;$ &   0.02 &    0.18 \\
NGC 6325 & 259.496708 & -23.766000 &    6.90 $\;\;\;\;$ &  &   31.67 $\pm \;$ &   1.77 &   -8.40 $\pm \;$ &   0.12 &   -9.06 $\pm \;$ &   0.10 &    0.19 \\
NGC 6333 & 259.796936 & -18.515943 &    7.90 $\;\;\;\;$ &  &  311.79 $\pm \;$ &   2.21 &   -2.20 $\pm \;$ &   0.03 &   -3.23 $\pm \;$ &   0.03 &    0.27 \\
NGC 6342 & 260.292000 & -19.587416 &    8.43 $\;\;\;\;$ &  &  116.50 $\pm \;$ &   0.80 &   -2.90 $\pm \;$ &   0.03 &   -7.09 $\pm \;$ &   0.03 &    0.10 \\
NGC 6356 & 260.895541 & -17.813027 &   15.10 $\;\;\;\;$ &  &   38.28 $\pm \;$ &   1.88 &   -3.86 $\pm \;$ &   0.04 &   -3.35 $\pm \;$ &   0.03 &    0.28 \\
NGC 6355 & 260.994125 & -26.353417 &    8.70 $\;\;\;\;$ &  & -194.67 $\pm \;$ &   1.48 &   -4.60 $\pm \;$ &   0.06 &   -0.47 $\pm \;$ &   0.05 &    0.29 \\
NGC 6352 & 261.371276 & -48.422168 &    5.89 $\;\;\;\;$ &  & -125.12 $\pm \;$ &   1.02 &   -2.18 $\pm \;$ &   0.02 &   -4.37 $\pm \;$ &   0.02 &    0.15 \\
IC 1257 & 261.785430 &  -7.093055 &   25.00 $\;\;\;\;$ &  & -138.78 $\pm \;$ &   2.13 &   -0.97 $\pm \;$ &   0.09 &   -1.39 $\pm \;$ &   0.07 &    0.11 \\
Ter 2 & 261.887916 & -30.802333 &    7.50 $\;\;\;\;$ &  &  131.32 $\pm \;$ &   1.18 &   -2.27 $\pm \;$ &   0.11 &   -6.19 $\pm \;$ &   0.10 &    0.21 \\
NGC 6366 & 261.934356 &  -5.079861 &    3.71 $\pm \;$ &   0.26 & -120.67 $\pm \;$ &   0.18 &   -0.39 $\pm \;$ &   0.02 &   -5.14 $\pm \;$ &   0.02 &    0.22 \\
Ter 4 & 262.662506 & -31.595527 &    7.20 $\;\;\;\;$ &  &  -48.00 $\pm \;$ &   1.73 &   -5.39 $\pm \;$ &   0.11 &   -3.33 $\pm \;$ &   0.09 &    0.05 \\
HP 1 & 262.771666 & -29.981666 &    6.80 $\;\;\;\;$ &  &   40.26 $\pm \;$ &   1.44 &    2.46 $\pm \;$ &   0.08 &  -10.17 $\pm \;$ &   0.07 &    0.13 \\
NGC 6362 & 262.979095 & -67.048332 &    7.30 $\pm \;$ &   0.31 &  -14.68 $\pm \;$ &   0.17 &   -5.49 $\pm \;$ &   0.01 &   -4.75 $\pm \;$ &   0.01 &   -0.04 \\
Lil 1 & 263.352333 & -33.389555 &    8.10 $\;\;\;\;$ &  &   59.95 $\pm \;$ &   2.62 &   -3.15 $\pm \;$ &   0.56 &   -5.32 $\pm \;$ &   0.41 &    0.64 \\
NGC 6380 & 263.616700 & -39.069200 &    9.80 $\;\;\;\;$ &  &   -7.51 $\pm \;$ &   2.30 &   -2.39 $\pm \;$ &   0.12 &   -3.22 $\pm \;$ &   0.10 &   -0.04 \\
Ter 1 & 263.946300 & -30.481000 &    6.70 $\;\;\;\;$ &  &   56.75 $\pm \;$ &   1.66 &   -2.87 $\pm \;$ &   0.09 &   -4.46 $\pm \;$ &   0.08 &    0.30 \\
Ton 2 & 264.043750 & -38.553333 &    6.40 $\;\;\;\;$ &  & -179.91 $\pm \;$ &   3.06 &   -5.58 $\pm \;$ &   0.13 &   -0.50 $\pm \;$ &   0.11 &    0.24 \\
NGC 6388 & 264.071777 & -44.735500 &   10.43 $\pm \;$ &   0.13 &   83.05 $\pm \;$ &   0.49 &   -1.32 $\pm \;$ &   0.02 &   -2.67 $\pm \;$ &   0.02 &    0.12 \\
NGC 6402 & 264.400391 &  -3.245917 &    9.18 $\pm \;$ &   0.46 &  -60.76 $\pm \;$ &   0.44 &   -3.65 $\pm \;$ &   0.02 &   -5.01 $\pm \;$ &   0.02 &    0.24 \\
NGC 6401 & 264.652500 & -23.909500 &    7.70 $\;\;\;\;$ &  &  -68.89 $\pm \;$ &   1.77 &   -2.76 $\pm \;$ &   0.07 &    1.50 $\pm \;$ &   0.06 &    0.15 \\
NGC 6397 & 265.175385 & -53.674335 &    2.47 $\pm \;$ &   0.04 &   18.51 $\pm \;$ &   0.08 &    3.31 $\pm \;$ &   0.01 &  -17.60 $\pm \;$ &   0.01 &   -0.18 \\
Pal 6 & 265.925833 & -26.222500 &    5.80 $\;\;\;\;$ &  &  186.80 $\pm \;$ &   2.30 &   -9.55 $\pm \;$ &   0.14 &   -5.39 $\pm \;$ &   0.12 &    0.40 \\
NGC 6426 & 266.227708 &   3.170138 &   20.60 $\;\;\;\;$ &  & -210.45 $\pm \;$ &   0.49 &   -1.81 $\pm \;$ &   0.03 &   -2.92 $\pm \;$ &   0.03 &    0.41 \\
Djor 1 & 266.867916 & -33.065555 &   13.70 $\;\;\;\;$ &  & -364.30 $\pm \;$ &   0.69 &   -3.58 $\pm \;$ &   0.09 &   -3.46 $\pm \;$ &   0.07 &   -0.04 \\
Ter 5 & 267.020200 & -24.779055 &    5.50 $\pm \;$ &   0.75 &  -82.83 $\pm \;$ &   0.93 &   -2.61 $\pm \;$ &   0.31 &   -5.00 $\pm \;$ &   0.29 &    0.33 \\
NGC 6440 & 267.219583 & -20.360250 &    8.24 $\;\;\;\;$ &  &  -67.49 $\pm \;$ &   0.93 &   -1.10 $\pm \;$ &   0.10 &   -3.71 $\pm \;$ &   0.09 &    0.41 \\
NGC 6441 & 267.554413 & -37.051445 &   11.83 $\pm \;$ &   0.13 &   16.54 $\pm \;$ &   0.96 &   -2.52 $\pm \;$ &   0.08 &   -5.48 $\pm \;$ &   0.08 &    0.11 \\
Ter 6 & 267.693250 & -31.275388 &    6.70 $\;\;\;\;$ &  &  136.89 $\pm \;$ &   1.69 &   -5.40 $\pm \;$ &   0.26 &   -7.08 $\pm \;$ &   0.22 &    0.20 \\
NGC 6453 & 267.715423 & -34.599166 &   11.60 $\;\;\;\;$ &  &  -94.94 $\pm \;$ &   2.02 &    0.27 $\pm \;$ &   0.03 &   -5.84 $\pm \;$ &   0.03 &    0.21 \\
UKS 1 & 268.613311 & -24.145277 &    7.80 $\;\;\;\;$ &  &   56.00 $\pm \;$ &   2.12 &   -2.59 $\pm \;$ &   0.52 &   -3.42 $\pm \;$ &   0.44 &    0.17 \\
NGC 6496 & 269.765350 & -44.265945 &   11.30 $\;\;\;\;$ &  & -134.56 $\pm \;$ &   0.23 &   -3.05 $\pm \;$ &   0.02 &   -9.22 $\pm \;$ &   0.02 &    0.05 \\
Ter 9 & 270.411666 & -26.839722 &    7.10 $\;\;\;\;$ &  &    6.85 $\pm \;$ &   3.07 &   -2.48 $\pm \;$ &   0.19 &   -7.45 $\pm \;$ &   0.16 &    0.19 \\
Djor 2 & 270.454583 & -27.825833 &    6.30 $\;\;\;\;$ &  &  -16.41 $\pm \;$ &   1.77 &    0.52 $\pm \;$ &   0.10 &   -3.06 $\pm \;$ &   0.09 &   -0.20 \\
NGC 6517 & 270.460500 &  -8.958777 &   10.60 $\;\;\;\;$ &  &  -40.06 $\pm \;$ &   0.49 &   -1.45 $\pm \;$ &   0.08 &   -4.22 $\pm \;$ &   0.08 &    0.30 \\
Ter 10 & 270.741666 & -26.072500 &    5.80 $\;\;\;\;$ &  &  -61.86 $\pm \;$ &   4.01 &   -6.88 $\pm \;$ &   0.08 &   -2.39 $\pm \;$ &   0.07 &    0.17 \\
NGC 6522 & 270.891750 & -30.033972 &    7.89 $\pm \;$ &   0.57 &  -14.89 $\pm \;$ &   0.66 &    2.63 $\pm \;$ &   0.05 &   -6.41 $\pm \;$ &   0.04 &    0.04 \\
NGC 6535 & 270.960449 &  -0.297639 &    6.50 $\;\;\;\;$ &  & -214.68 $\pm \;$ &   0.39 &   -4.25 $\pm \;$ &   0.03 &   -2.92 $\pm \;$ &   0.03 &    0.02 \\
NGC 6528 & 271.206833 & -30.056277 &    7.45 $\;\;\;\;$ &  &  211.60 $\pm \;$ &   0.81 &   -2.16 $\pm \;$ &   0.09 &   -5.63 $\pm \;$ &   0.08 &    0.13 \\
NGC 6539 & 271.207000 &  -7.585861 &    8.40 $\;\;\;\;$ &  &   35.25 $\pm \;$ &   0.53 &   -6.67 $\pm \;$ &   0.07 &   -3.33 $\pm \;$ &   0.06 &    0.18 \\
NGC 6540 & 271.535833 & -27.765277 &    5.20 $\;\;\;\;$ &  &  -17.22 $\pm \;$ &   0.94 &   -3.79 $\pm \;$ &   0.08 &   -2.80 $\pm \;$ &   0.07 &    0.16 \\
NGC 6544 & 271.835750 & -24.997333 &    2.57 $\pm \;$ &   0.37 &  -38.41 $\pm \;$ &   0.71 &   -2.26 $\pm \;$ &   0.09 &  -18.68 $\pm \;$ &   0.09 &    0.13 \\
NGC 6541 & 272.009826 & -43.714889 &    8.24 $\pm \;$ &   0.41 & -164.05 $\pm \;$ &   0.44 &    0.33 $\pm \;$ &   0.01 &   -8.83 $\pm \;$ &   0.01 &   -0.20 \\
ESO 280-SC06   & 272.275000 & -46.423333 &   22.90 $\;\;\;\;$ &  &   92.94 $\pm \;$ &   0.30 &   -0.57 $\pm \;$ &   0.06 &   -2.75 $\pm \;$ &   0.04 &    0.26 \\
\hline
\end{tabular}
\label{tabpm}
\end{table*}

\begin{table*}
\contcaption{}
\begin{tabular}{lrrr@{}lr@{}lr@{}lr@{}lr}
\hline
 & & & & & & & & \\[-0.3cm]
\multirow{2}{*}{Name} &  \multicolumn{1}{c}{RA} & \multicolumn{1}{c}{DEC} & \multicolumn{2}{c}{$R_\odot$} & \multicolumn{2}{c}{$R_V$} &\multicolumn{2}{c}{$\mu_\alpha \cos \delta$} & \multicolumn{2}{c}{$\mu_\delta$} & \multirow{2}{*}{$\rho_{\mu_\alpha \mu_\delta}$}  \\
 &  \multicolumn{1}{c}{$[^0]$} & \multicolumn{1}{c}{$[^0]$} & \multicolumn{2}{c}{[kpc]} & \multicolumn{2}{c}{[km/sec]} & \multicolumn{2}{c}{[mas/yr]} & \multicolumn{2}{c}{[mas/yr]} & \\[+0.1cm]
\hline
 & & & & & & & & \\[-0.3cm]
NGC 6553 & 272.323333 & -25.908694 &    6.46 $\pm \;$ &   0.44 &    0.27 $\pm \;$ &   0.37 &    0.34 $\pm \;$ &   0.06 &   -0.42 $\pm \;$ &   0.06 &    0.15 \\
2MS 2 & 272.402099 & -20.778888 &    4.90 $\;\;\;\;$ &  & -237.75 $\pm \;$ &  10.10 &   -0.76 $\pm \;$ &   0.14 &   -2.22 $\pm \;$ &   0.13 &    0.64 \\
NGC 6558 & 272.573333 & -31.763888 &    7.40 $\;\;\;\;$ &  & -195.19 $\pm \;$ &   0.67 &   -1.75 $\pm \;$ &   0.03 &   -4.12 $\pm \;$ &   0.03 &    0.08 \\
IC 1276 & 272.684166 &  -7.207611 &    5.38 $\pm \;$ &   0.51 &  155.04 $\pm \;$ &   0.69 &   -2.48 $\pm \;$ &   0.03 &   -4.39 $\pm \;$ &   0.03 &    0.17 \\
Ter 12 & 273.065833 & -22.741944 &    4.80 $\;\;\;\;$ &  &   93.69 $\pm \;$ &   0.89 &   -5.92 $\pm \;$ &   0.08 &   -2.70 $\pm \;$ &   0.07 &    0.30 \\
NGC 6569 & 273.411666 & -31.826888 &   10.60 $\pm \;$ &   0.78 &  -49.88 $\pm \;$ &   0.42 &   -4.14 $\pm \;$ &   0.03 &   -7.29 $\pm \;$ &   0.03 &    0.12 \\
BH 261 & 273.527500 & -28.635000 &    6.50 $\;\;\;\;$ &  &  -31.87 $\pm \;$ &   3.83 &    3.60 $\pm \;$ &   0.04 &   -3.55 $\pm \;$ &   0.04 &    0.37 \\
NGC 6584 & 274.656646 & -52.215778 &   13.18 $\;\;\;\;$ &  &  259.75 $\pm \;$ &   1.55 &   -0.05 $\pm \;$ &   0.02 &   -7.21 $\pm \;$ &   0.02 &   -0.08 \\
Mercer 5 & 275.832500 & -13.668611 &    5.50 $\;\;\;\;$ &  &  &  &   -4.42 $\pm \;$ &   0.24 &   -6.36 $\pm \;$ &   0.21 &    0.19 \\
NGC 6624 & 275.918793 & -30.361029 &    6.64 $\pm \;$ &   0.42 &   53.39 $\pm \;$ &   0.95 &    0.09 $\pm \;$ &   0.03 &   -6.90 $\pm \;$ &   0.03 &    0.01 \\
NGC 6626 & 276.136708 & -24.869778 &    5.55 $\pm \;$ &   0.35 &   10.85 $\pm \;$ &   0.51 &   -0.34 $\pm \;$ &   0.02 &   -8.89 $\pm \;$ &   0.02 &   -0.37 \\
NGC 6638 & 277.733734 & -25.497472 &   10.32 $\;\;\;\;$ &  &   12.26 $\pm \;$ &   1.36 &   -2.55 $\pm \;$ &   0.02 &   -4.05 $\pm \;$ &   0.02 &    0.37 \\
NGC 6637 & 277.846252 & -32.348083 &    8.80 $\;\;\;\;$ &  &   48.56 $\pm \;$ &   1.28 &   -5.10 $\pm \;$ &   0.01 &   -5.81 $\pm \;$ &   0.01 &    0.40 \\
NGC 6642 & 277.975416 & -23.475194 &    8.05 $\;\;\;\;$ &  &  -34.32 $\pm \;$ &   0.86 &   -0.21 $\pm \;$ &   0.03 &   -3.89 $\pm \;$ &   0.03 &    0.14 \\
NGC 6652 & 278.940124 & -32.990722 &   10.00 $\;\;\;\;$ &  &  -95.04 $\pm \;$ &   2.19 &   -5.50 $\pm \;$ &   0.02 &   -4.22 $\pm \;$ &   0.02 &    0.00 \\
NGC 6656 & 279.099762 & -23.904749 &    3.23 $\pm \;$ &   0.08 & -147.89 $\pm \;$ &   0.28 &    9.83 $\pm \;$ &   0.01 &   -5.54 $\pm \;$ &   0.01 &    0.21 \\
Pal 8 & 280.374572 & -19.825834 &   12.80 $\;\;\;\;$ &  &  -18.53 $\pm \;$ &   5.73 &   -2.06 $\pm \;$ &   0.02 &   -5.63 $\pm \;$ &   0.02 &    0.33 \\
NGC 6681 & 280.803162 & -32.292110 &    9.35 $\pm \;$ &   0.18 &  216.88 $\pm \;$ &   0.89 &    1.41 $\pm \;$ &   0.02 &   -4.72 $\pm \;$ &   0.02 &    0.29 \\
NGC 6712 & 283.267916 &  -8.706111 &    7.08 $\pm \;$ &   0.41 & -107.65 $\pm \;$ &   0.29 &    3.33 $\pm \;$ &   0.01 &   -4.39 $\pm \;$ &   0.01 &    0.19 \\
NGC 6715 & 283.763855 & -30.479862 &   23.81 $\pm \;$ &   0.34 &  142.71 $\pm \;$ &   0.55 &   -2.73 $\pm \;$ &   0.03 &   -1.41 $\pm \;$ &   0.03 &    0.21 \\
NGC 6717 & 283.775177 & -22.701473 &    7.10 $\;\;\;\;$ &  &   28.61 $\pm \;$ &   0.58 &   -3.10 $\pm \;$ &   0.03 &   -4.97 $\pm \;$ &   0.03 &    0.52 \\
NGC 6723 & 284.888123 & -36.632248 &    8.08 $\pm \;$ &   0.43 &  -94.36 $\pm \;$ &   0.26 &    1.00 $\pm \;$ &   0.01 &   -2.44 $\pm \;$ &   0.01 &    0.13 \\
NGC 6749 & 286.313750 &   1.884166 &    7.80 $\;\;\;\;$ &  &  -58.43 $\pm \;$ &   0.86 &   -2.89 $\pm \;$ &   0.07 &   -6.01 $\pm \;$ &   0.07 &    0.26 \\
NGC 6752 & 287.717102 & -59.984554 &    4.20 $\pm \;$ &   0.09 &  -26.36 $\pm \;$ &   0.15 &   -3.19 $\pm \;$ &   0.02 &   -4.00 $\pm \;$ &   0.02 &    0.13 \\
NGC 6760 & 287.800041 &   1.030472 &    7.40 $\;\;\;\;$ &  &   -1.25 $\pm \;$ &   1.22 &   -1.18 $\pm \;$ &   0.04 &   -3.59 $\pm \;$ &   0.04 &    0.34 \\
NGC 6779 & 289.148193 &  30.183471 &   10.38 $\pm \;$ &   0.79 & -137.47 $\pm \;$ &   0.46 &   -2.01 $\pm \;$ &   0.02 &    1.70 $\pm \;$ &   0.02 &    0.05 \\
Ter 7 & 289.432983 & -34.657722 &   22.80 $\;\;\;\;$ &  &  159.58 $\pm \;$ &   0.14 &   -2.98 $\pm \;$ &   0.03 &   -1.58 $\pm \;$ &   0.03 &    0.29 \\
Pal 10 & 289.508728 &  18.571666 &    5.90 $\;\;\;\;$ &  &  -31.21 $\pm \;$ &   0.35 &   -4.20 $\pm \;$ &   0.11 &   -7.04 $\pm \;$ &   0.10 &    0.06 \\
Arp 2 & 292.183807 & -30.355638 &   28.60 $\;\;\;\;$ &  &  122.79 $\pm \;$ &   0.32 &   -2.39 $\pm \;$ &   0.03 &   -1.53 $\pm \;$ &   0.03 &    0.12 \\
NGC 6809 & 294.998779 & -30.964750 &    5.60 $\pm \;$ &   0.26 &  174.56 $\pm \;$ &   0.19 &   -3.41 $\pm \;$ &   0.01 &   -9.26 $\pm \;$ &   0.01 &    0.11 \\
Ter 8 & 295.435028 & -33.999474 &   26.73 $\;\;\;\;$ &  &  148.48 $\pm \;$ &   0.16 &   -2.44 $\pm \;$ &   0.02 &   -1.56 $\pm \;$ &   0.01 &   -0.25 \\
Pal 11 & 296.310000 &  -8.007222 &   14.30 $\;\;\;\;$ &  &  -68.26 $\pm \;$ &   0.96 &   -1.77 $\pm \;$ &   0.06 &   -4.91 $\pm \;$ &   0.05 &    0.31 \\
NGC 6838 & 298.443726 &  18.779194 &    3.65 $\pm \;$ &   0.26 &  -22.33 $\pm \;$ &   0.18 &   -3.41 $\pm \;$ &   0.02 &   -2.60 $\pm \;$ &   0.02 &    0.15 \\
NGC 6864 & 301.519541 & -21.921166 &   21.61 $\pm \;$ &   1.02 & -188.13 $\pm \;$ &   1.00 &   -0.58 $\pm \;$ &   0.02 &   -2.79 $\pm \;$ &   0.02 &    0.24 \\
NGC 6934 & 308.547393 &   7.404472 &   15.40 $\pm \;$ &   0.58 & -406.25 $\pm \;$ &   0.66 &   -2.65 $\pm \;$ &   0.02 &   -4.69 $\pm \;$ &   0.01 &    0.26 \\
NGC 6981 & 313.365417 & -12.537305 &   17.00 $\;\;\;\;$ &  & -331.39 $\pm \;$ &   1.47 &   -1.30 $\pm \;$ &   0.02 &   -3.32 $\pm \;$ &   0.02 &    0.40 \\
NGC 7006 & 315.372416 &  16.187333 &   58.80 $\;\;\;\;$ &  & -383.02 $\pm \;$ &   0.69 &   -0.06 $\pm \;$ &   0.04 &   -0.62 $\pm \;$ &   0.04 &   -0.11 \\
NGC 7078 & 322.493042 &  12.167001 &   10.22 $\pm \;$ &   0.13 & -106.74 $\pm \;$ &   0.23 &   -0.63 $\pm \;$ &   0.01 &   -3.80 $\pm \;$ &   0.01 &   -0.10 \\
NGC 7089 & 323.362579 &  -0.823250 &   10.87 $\pm \;$ &   0.47 &   -3.51 $\pm \;$ &   0.34 &    3.50 $\pm \;$ &   0.01 &   -2.17 $\pm \;$ &   0.01 &    0.01 \\
NGC 7099 & 325.092133 & -23.179861 &    8.69 $\pm \;$ &   0.11 & -185.29 $\pm \;$ &   0.14 &   -0.72 $\pm \;$ &   0.01 &   -7.24 $\pm \;$ &   0.01 &    0.53 \\
Pal 12 & 326.661804 & -21.252611 &   19.00 $\;\;\;\;$ &  &   27.99 $\pm \;$ &   0.25 &   -3.28 $\pm \;$ &   0.03 &   -3.31 $\pm \;$ &   0.03 &    0.33 \\
Pal 13 & 346.685166 &  12.772000 &   24.80 $\;\;\;\;$ &  &   25.95 $\pm \;$ &   0.30 &    1.97 $\pm \;$ &   0.11 &    0.28 $\pm \;$ &   0.08 &   -0.03 \\
NGC 7492 & 347.110958 & -15.611500 &   26.55 $\;\;\;\;$ &  & -176.81 $\pm \;$ &   0.26 &    0.77 $\pm \;$ &   0.03 &   -2.28 $\pm \;$ &   0.03 &    0.10 \\
\hline
\end{tabular}
\end{table*}


